Cross-modal Learning of Graph Representations using Radar Point Cloud for Long-Range Gesture Recognition

Gesture recognition is one of the most intuitive ways of interaction and has gathered particular attention for human computer interaction. Radar sensors possess multiple intrinsic properties, such as their ability to work in low illumination, harsh weather conditions, and being low-cost and compact, making them highly preferable for a gesture recognition solution. However, most literature work focuses on solutions with a limited range that is lower than a meter. We propose a novel architecture for a long-range (1m - 2m) gesture recognition solution that leverages a point cloud-based cross-learning approach from camera point cloud to 60-GHz FMCW radar point cloud, which allows learning better representations while suppressing noise. We use a variant of Dynamic Graph CNN (DGCNN) for the cross-learning, enabling us to model relationships between the points at a local and global level and to model the temporal dynamics a Bi-LSTM network is employed. In the experimental results section, we demonstrate our model's overall accuracy of 98.4% for five gestures and its generalization capability.

==> background.tex <==
In this section, we provide some background on Point Clouds and \acp{gnn}.
Point Clouds are a sparse and unordered set of points in space, typically containing information about the 3D shape of objects in Cartesian space.

Since traditional neural network structures like \acp{cnn} and \acp{fcn} are efficient only on regular grids and not invariant to input permutations, they are not well suited for point cloud processing.
\acp{gnn} on the other hand, are equivariant to input permutations and do not require points on regular grids. Point clouds can directly be represented as a graph structure by looking at them as a set of nodes with corresponding feature vectors, made up by Cartesian coordinates and possibly other features like velocity and edges containing distance- and structural information. Similar to traditional neural networks, \acp{gnn} then build up compressed representations, embeddings, of the inputs, which may contain information about local structures and higher-level features.
In this work, we used a novel operation named EdgeConv \cite{wang2019dynamic}. Overall, EdgeConv learns the embeddings of the relationships between a point and its neighbors while simultaneously being permutation invariant. A more detailed definition and how we integrated EdgeConv into our network can be found in section \ref{section:edgeconv}







%In this section we provide some background on Point Clouds and \acp{gnn}.
%Point Clouds are a sparse and unordered set of points in space, typically containing information about the 3D-shape of objects in Cartesian space.
%%that can also contain a lot of information about corresponding object. %Because of their unparticular order, their global structure is inherently non-Euclidean. 
%Since point clouds do not have regular grids, processing this information-rich data structure with traditional neural networks, such as \acp{cnn}, is difficult and may cause the loss of some topological information \cite{wang2019dynamic}.
%%In a recent dominant approach of learning on point clouds, which we also used in this work \cite{wang2019dynamic}, a graph is used as a compact representation of a point cloud and a novel simple operation is proposed that operates in the sense of \ac{gnn}.
%Morever, since point clouds do not have a fixed order, performing operations on point clouds should be invariant to the node ordering or permutation.
%\acp{gnn} are proposed to process the graph structured data without changing its structure and also to take advantage of its benefits. It performs by learning the embedding features of the nodes, which also contain the information about the neighboring nodes, and iteratively updating these features by aggregating them along the edges \cite{2021}. There are two important features of \acp{gnn} that give us an advantage over other \acrfull{ml} methods that use regular grid-structured data as input: permutation invariance and permutation equivariance. %In a graph structured data, the nodes have no particular order. 
%Instead of repeatedly sampling and ordering the nodes of the graphs, we construct the graph once and with the permutation invariance property of \acp{gnn}, we ensure that we get the same results for any isomorphic graphs. 
%Besides, the permutation equivariance property allows us to determine which part of the output belongs to which part of the graph, i.e., the granularity.
%In this work, we used a novel simple operation named EdgeConv \cite{wang2019dynamic}, which operates in the sense of \acp{gnn}. Overall, EdgeConv learns the embeddings of the relationships between a point and its neighbors while simultaneously beeing permutation invariant. A more detailed definition and how we integrated EdgeConv into our network can be found in section \ref{section:edgeconv}




%%%%%%%
%Points are irregular, meaning that if we take a point and permute it, the spatial distribution of the point cloud would not change. In order to preserve the irregularity of non-Euclidean and exploit their structure, there are some proposed neural networks to process non-Euclidean data without loss of information

%In the novel approach proposed in \cite{wang2019dynamic}, as mentioned above, a local directed %neighborhood graph $G=(V,E)$ with self-loop is constructed from the k-nearest neighbor (k-NN) graph of a point cloud with n points, labeled $X = \{x_1,...,x_n\}$. On the edge features of $G$ defined as $\mathbf{e}_{ij}=\mathbf{h}_{\Theta}(\mathbf{x}_i,\mathbf{x}_j)$, with $\mathbf{h}_{\Theta}$ being a differentiable non-linear function with learnable parameters $\mathbf{\Theta}$, the novel proposed simple operation called EdgeConv  applied. The output of the EdgeConv at the $i$-th node is calculated as follows
%\begin{equation} \label{EdgeConv output}
%\mathbf{{x}^{'}}_{i} = \underset{j:(i,j)\in E}{\square} %\mathbf{h}_{\Theta}(\mathbf{x}_i,\mathbf{x}_j),
%\end{equation}
%where $\square$ is channelwise symmetric aggregation operation. Overall, EdgeConv learns the embeddings of the relationships between a point and its neighbors while simultaneously beeing permutation invariant. After each EdgeConv block, the graph is dynamically updated, which is a significant difference from previous graph CNNs.
